Homogenizable structures and model completeness

A homogenizable structure $\mathcal{M}$ is a structure where we may add a finite amount of new relational symbols to represent some $\emptyset-$definable relations in order to make the structure homogeneous. In this article we will divide the homogenizable structures into different classes which categorize many known examples and show what makes each class important. We will show that model completeness is vital for the relation between a structure and the amalgamation bases of its age and give a necessary and sufficient condition for an $\omega-$categorical model-complete structure to be homogenizable.

==> modelcompleteness.tex <==
\begin{defi}\label{SEAPdef}
Let $\mbK$ be a set of finite structures and $k,m\in \mbbN$ and define the $(k,m)$ sub extension amalgamation failure property (SEAP$_{k,m}$) to be the following. For any $\mcA,\mcB,\mcC\in \mbK$ with embeddings $f:\mcA\rightarrow\mcB,g:\mcA\rightarrow \mcC$ without an amalgam, there exists $\mcA_0\subseteq \mcA$, $\mcB_0\supseteq \mcB$ and $\mcC_0\supseteq \mcC$ with $|A_0|<k$, $|B_0|-|B|<m$ and $|C_0|-|C|<m$ such that $f_0:\mcA_0\rightarrow \mcB_0$ and $g_0:\mcA_0\rightarrow\mcC_0$ with $f_0=f\reduct_{A_0}$ and $g_0=g\reduct_{A_0}$does not have an amalgam. \\\indent  We say that $\mbK$ satisfies SEAP if it satisfies SEAP$_{k,m}$ for some $k,m\in\mbbN$.
\end{defi}

\begin{lma} Let $\mcM$ be a structure such that the model companion $\mcN$ is $\omega-$categorical. If $Age(\mcM)$ satisfies SEAP then $\mcN$ is homogenizable.
\end{lma}
\begin{proof}
Let $m$ and $k$ be numbers such that $Age(\mcM)$ satisfies SEAP$_{k,m}$. As $\mcN$ is $\omega-$categorical there are only a finite amount of types of the tuples of size less than $k$. Let $V'\supseteq V$ be a the extended vocabulary where, for each $i<k$, and $i-$type over $\emptyset$ there is an $i-$ary new relational symbol. Let $\overline \mcN$ be the $V'-$structure such that $\mcN = \overline \mcN \reduct V$ and for each relational symbol $R$ in $V'-V$ there is a complete type $p(\bar x)$ over $\emptyset$ in $\mcN$ such that for each $\bar a \in N$, $\mcN\models p(\bar a)$ if and only if $\overline \mcN\models R(\bar a)$. Thus the new relational symbols isolates the $1-$, $2-,...,(k-2)-$ and $(k-1)-$types in $\mcN$ and as $\mcN$ is $\omega-$categorical these relations are $\emptyset-$definable. We claim that $\overline \mcN$ is homogeneous, and thus $\mcN$ was homogenizable.\\\indent
In search for a contradiction, assume that $\overline \mcN$ is not homogeneous, thus there exists tuples $\bar a,\bar b\in \overline N$ with the same atomic diagram such that $tp^{\overline \mcN}(\bar a)\neq tp^{\overline \mcN}(\bar b)$. As $\bar N$ is just an expansion of $\emptyset-$definable relations, it follows that $tp^\mcN(\bar a) \neq tp^\mcN(\bar b)$. The model completeness and $\omega-$categoricity of $\mcN$ implies that all types are isolated by $\Sigma_1-$formulas. Let $\bar a_0$ and $\bar b_0$ be tuples such that all existensial quantifiers of all types of $\bar a$ and $\bar b$ respectively are witnessed by subtuples of $\bar a_0$ and $\bar b_0$ respectively. Let $\mcA = \mcN\reduct \bar a, \mcB = \mcN\reduct \bar b\bar b_0, \mcC = \mcN \reduct \bar a\bar a_0$, and note that since $tp(\bar a)\neq tp(\bar b)$ the diagram created by the inclusion embeddings with $\mcA,\mcB$ and $\mcC$ can not have an amalgam. As $Age(\mcM)= Age(\mcN)$ satisfies SEAP$_{k,m}$ there exists $\mcA_0\subseteq \mcA, \mcB_0\supseteq \mcB$ and $\mcC_0\supseteq \mcC$ such that $|A_0|<k$ and the induced diagram does not have an amalgam. This in turn implies there are embeddings $f:\mcB_0\rightarrow \mcN, g:\mcC_0\rightarrow \mcN$ such that $tp(f(A_0)) \neq tp(g(A_0))$. However both $\bar a$ and $\bar b$ had the same atomic diagram in $\overline mcN$, and thus all tubtuples of size less than $k$ have the same type. As $\mcB_0$ and $\mcC_0$ contained witnesses for all isolating formulas of all types in $\mcA$ we conclude that $tp(f(A_0))=tp(g(A_0))$ has to hold, which is a contradiction.  
\end{proof}
\begin{lma}
If $\mcM$ is a homogenizable model complete structure then $\mcM$ is $\Sigma_1-$homogenizable, with all types isolated by the $\Sigma_1-$homogenization and if $\mcM$ is not homogeneous then $Age(\mcM)$ satisfies SEAP.
\end{lma}
\begin{proof}
Model completeness is equivalent with that each formula is equivalent to a $\Sigma_1-$formula. Hence the types may be assumed to be isolated by $\Sigma_1-$formulas, so taking the disjunction which describes tuples satisfying a certain homogenizing formula will create $\Sigma_1-$formulas which are equivalent with the homogenizing formulas. \\\indent 
In order to prove the last property assume that $Age(\mcM)$ does not satisfy AP. Let $\mcA,\mcB,\mcC\in Age(\mcM)$ with embeddings $f:\mcA\rightarrow \mcB$, $g:\mcA\rightarrow \mcC$ be without an amalgam. We conclude that $tp(f(A))\neq tp(g(A))$, however since they have the same atomic diagram there has to exist homogenizing formulas $\exists \bar y\varphi(\bar x,\bar y),\exists \bar y \psi(\bar x,\bar y)$ such that for some $\bar a_0\in A$, $\mcM\models \exists \bar y\varphi (f(\bar a_0),\bar y)\wedge \neg \exists \bar y\varphi(g(\bar a_0),\bar y) \wedge \neg \exists \bar y \psi(f(\bar a_0),\bar y)\wedge \exists \bar y \psi(g(\bar a_0),\bar y)$. Note that we may assume
\begin{equation}\label{eq1}\mcM\models \forall \bar x (\exists \bar y\varphi(\bar x, \bar y) \leftrightarrow \neg \exists \bar y \psi(\bar x,\bar y) )
\end{equation}
Let $\mcA_0 = \mcA\reduct {\bar a}$, let $\mcB_0$ be $\mcB$ extended with the tuple witnessing $\exists \bar y\varphi(f(\bar a),\bar y)$ and let $\mcC_0$ be $\mcC$ extended with the tuple witnessing $\exists \bar y\varphi(g(\bar a),\bar y)$. Then $f_0: \mcA_0\rightarrow \mcB_0$, $f_0 = f\reduct_{A_0}$ and $g_0:\mcA_0\rightarrow \mcC_0$, $g_0 = g\reduct_{A_0}$ can not have an amalgam since (\ref{eq1}) hold and $\mcM\models \exists \bar y\varphi(f_0(\bar a),\bar y) \wedge \exists \bar y \psi(g_0(\bar a),\bar y)$.
%$\Sigma_1-$formulas in $\mcM$ we may extend $\mcB$ and $\mcC$ into tuples $\mcC_0,\mcB_0$ witnessing the formulas which isolates the type of some tuple in the image of $\mcA$. Let $\mcA_0$ be the restriction of $\mcA$ to that single tuple. 
%Then $Diag(\mcA_0;\mcB_0,\mcC_0)$ can not have an amalgam, since the type of the image of $\mcA_0$ could then not be determined.
\end{proof}
Combining the previous two lemmas we now have a proof for Theorem \ref{mcmainthm}.
In \cite{C} Covington asks whether all homogenizable classes have a homogenizable model companion. By the previous theorem it is clear that we can find a homogenizable class without a homogenizable model companion if and only if there is a homogenizable class not satisfying SEAP. The author does not know whether such a class exists and hence the question remains open. 

